From Bi-Level to One-Level: A Framework for Structural Attacks to Graph Anomaly Detection

The success of graph neural networks stimulates the prosperity of graph mining and the corresponding downstream tasks including graph anomaly detection (GAD). However, it has been explored that those graph mining methods are vulnerable to structural manipulations on relational data. That is, the attacker can maliciously perturb the graph structures to assist the target nodes to evade anomaly detection. In this paper, we explore the structural vulnerability of two typical GAD systems: unsupervised FeXtra-based GAD and supervised GCN-based GAD. Specifically, structural poisoning attacks against GAD are formulated as complex bi-level optimization problems. Our first major contribution is then to transform the bi-level problem into one-level leveraging different regression methods. Furthermore, we propose a new way of utilizing gradient information to optimize the one-level optimization problem in the discrete domain. Comprehensive experiments demonstrate the effectiveness of our proposed attack algorithm BinarizedAttack.

==> sections/acknowledgement.tex <==
\section{Acknowledgement}
The work is supported by Secure \& Trustworthy Intelligence Laboratory (STiL) established by Prof. Kai Zhou.

==> sections/defence.tex <==
\section{Possible Countermeasures}
\label{sec-defense}
Defense approaches against data poisoning attacks have been extensive studied mainly in the computer vision domain. Typical methods include sanitizing the dataset by identifying and removing the maliciously injected data points, training robust models that could still perform well on poisoned data, and so on. More recently, there are also works that explore defense approaches in the graph learning domain. 
%Defence against the adversarial examples have been widely explored in recent years. The defence method is firstly implemented on the image classification field. The image data are continuous and it is easy to craft unnoticeable perturbations on the image field. \cite{DBLP:journals/corr/abs-1711-01991} introduced the randomization and smoothing technique to increase the robustness of the deep convolutional neural networks.\cite{Tramer} tended to generated the adversarial examples into the training data to enhance the vulnerable model. 
For example, based on the observation that $\mathsf{netattack}$ \cite{Z_gner_2018} tends to increase the rank of the adjacency matrix, \cite{10.1145/3336191.3371789} proposed the low-rank approximation of the adjacency matrix by SVD for defense. Graph variational autoencoder is used in \cite{DBLP:journals/corr/abs-2006-08900} to generate a smooth adjacency matrix to defend two popular attacks $\mathsf{metattack}$\cite{DBLP:journals/corr/abs-1902-08412} and $\mathsf{netattack}$. A robust GCN~\cite{kipf2017semisupervised} model is proposed in \cite{zhu2019robust} by formulating the Gaussian distribution based on the hidden features of GCN and penalizing the high variance to enhance the robustness. \cite{DBLP:journals/corr/abs-1908-07558} and \cite{DBLP:journals/corr/abs-2006-08149} introduced the attention mechanism to decrease the effect of adversarial links in the attacked graph.



In this paper, we further explore possible countermeasures to defend against $\mathsf{BinarizedAttack}$. Our key observation is that, since OLS \cite{Zdaniuk2014} estimation  is sensitive to poisoned data in the training process, we can use robust estimators  instead to estimate the regression parameters. Huber \cite{10.1214/aoms/1177703732} proposed the Huber loss function to replace the mean square loss:
\begin{equation}
\rho_{Huber}(t)=\left\{
\begin{aligned}
&\frac{1}{2}t^{2},\quad  \text{if} \ |t|\leq k, \\
&k|t|-\frac{1}{2}k^{2}, \quad \text{if} \ |t| > k.
\end{aligned}
\right.
\end{equation}
where $k$ is the hyper-parameter to penalize the outliers linearly instead of quadratically.

Random Sample Consensus (RANSAC \cite{ransac}) uses Huber loss with $k=1$ for robust estimation.
It was known that RANSAC is able to estimate the model parameters that achieve high accuracy even when the dataset contains a significant number of outliers. In light of this, we adopt the robust estimation method from  RANSAC to estimate the parameters of $\mathsf{OddBall}$ (thus a robust version of $\mathsf{OddBall}$) from the poisoned graph generated by $\mathsf{BinarizedAttack}$. Our experiments show that this robust estimation approach can slightly mitigate the attack effect. The defense of structural poisoning attack remains as an important future work.


%For example, if $k=1$ the Huber loss curve is 
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale=0.7]{figures/Huber.png}
%	\caption{Green line is Huber loss with $k=1$, blue line is $\frac{1}{2}t^{2}$}
%\end{figure}
%Random sample consensus (RANSAC \cite{ransac}) is an iterative method to estimate the parameters of the model whose training dataset contains outliers, it is an outlier detection method. The advantage of {RANSAC} is that it can estimate the parameters with high accuracy even when the dataset contains a significant number of outliers.

==> sections/targetLGCN.tex <==
\section{Black-box Attacks Against GCN-Based Anomaly Detection}
\label{sec-black-box-attack}
\subsection{Attack Model}


==> sections/transfer.tex <==
\section{Attack Transferability}
\label{sec-transfer}
In this section, we investigate the attack transferability of $\mathsf{BinarizedAttack}$ to two other GAD systems that are based on representation learning.

\subsection{Representation-learning-based GAD}
Recently, graph analysis based on representation learning has attracted extensive research attention. Graph representation learning~\cite{hamilton2020graph} aims to learn a low-dimensional latent vector for each node (called embedding) that could capture the feature as well as the structural information of the graph. Those learned embeddings are then used in a wide range of down-stream tasks such as node classification and link prediction. Following this trend, graph representation learning has also been used as the core technique for anomaly detection. These techniques entitle the defender the freedom to choose different GAD systems in practice, which raises a practical question: could an attack method that is specifically designed for a target GAD system be effective to other GAD systems? We investigate this problem of attack transferability by using $\mathsf{BinarizedAttack}$ to attack two other GAD systems (GAL~\cite{10.1145/3340531.3411979} and ReFeX~\cite{ReFeX}) based on graph representation learning.

At a high level, representation-learning-based GAD systems have two components: representation learning and classification. First, given a graph as input, the system learns the embeddings of nodes using various methods (e.g., graph neural networks, random walk, etc.). These embeddings are then fed into classifiers such as Multi-Layer Perceptron (MLP) which will classify nodes as anomalous or benign. These GAD systems differ mainly in the methods used for learning the node embeddings. We focus on two representative systems as below.

\subsubsection{GAL~\cite{10.1145/3340531.3411979}} GAL utilizes Graph Neural Networks \cite{kipf2017semisupervised} (GNNs) to learn the node embeddings. In particular, GAL replaced the loss function in typical GNNs with a \textit{graph anomaly loss} that is specially designed for anomaly detection. It is a class-distribution-aware margin loss which solves the imbalanced problem in anomaly detection via automatically adjusting the margins for the minority class (i.e., anomaly). Specifically, the loss on node $u$ is computed as:

\begin{align}
\mathcal{L}(u)=&E_{u_{+}\sim \mathcal{U}_{u+},u_{-}\sim \mathcal{U}_{u-}} max\{0,g(u,u_{-})-g(u,u_{+})+\Delta_{y_{u}}\}, \nonumber \\
&\text{where} \quad \Delta_{y_{u}}=\frac{C}{n_{y_{u}}^{1/4}}. \label{eqn-gal}
\end{align}
Here $\mathcal{U}_{u+}$ denotes the set of nodes share the same label with $u$, and vice versa. $g(u,u^{\prime})=f(u)^{T}f(u^{\prime})$ measures the similarity of the representation of two nodes $u$ and $u^{\prime}$, $f$ is the GNN. $C$ is the constant hyperparameter to be tuned. $\Delta_{y_{u}}$ is proved to best weigh up between the improvement of the generalization of minority class and the sub-optimal margin for the frequent class.
%{\color{red} explain this loss function to make it self-contained!}
%In this section we present the mechanism of transfer attack to other embedding-based anomaly detection, i.e., GAL \cite{10.1145/3340531.3411979} and ReFeX \cite{ReFeX}. Both of them have two vital systems: representation learning and classification. In the representation learning part, GAL and ReFeX learn the embeddings for each node in the graph with the aid of their own algorithm. The learned embeddings contains important structural informations in the graph. In the classification part, we implement a strong classifier like multi-layer perceptron (MLP) to measure the quality of embeddings for the anomaly detection in supervised manner. High AUC or F1 score stand for the saying that the embeddings indeed capture the hidden structural informations which can distinguish out the nodes with anomaly structure in graph. We focus on the adversarial robustness on the embedding space of GAL and ReFeX, that is, we measure the robustness of the embeddings itself rather than the classification accuracy of the downstream tasks against $\mathsf{BinarizedAttack}$. 

%{\color{red} we want to measure the quality of representation by its adversarial robustness (instead of just the accuracy of downstream tasks) -- robust features.}

\subsubsection{ReFeX~\cite{ReFeX}}
ReFeX (Recursive Feature eXtraction) is a novel algorithm that combines node-based local features with neighborhood (ego-based) features recursively, and output regional features which can capture the behavior information in large social networks. ReFeX aggregates the local and ego-based features and use them to create recursive features. Local features are essentially node degree measures. Egonet features are $\mathbf{N}$ and $\mathbf{E}$ as mentioned in Section III. ReFeX recurses the local and ego-based features by calculating their means and sums. Next ReFeX implements the pruning method using \textit{vertical logarithmic binning}. At last, ReFeX transforms the pruned recursive features to binary-valued embeddings. The pruned recursive features proved to efficiently capture the inner structural information provided by the graph. In this paper, we make use of these features for node anomaly detection.

\subsection{Transfer attack methodology}
\label{sec-transfer-method}
%In the transfer attack experiments, we simultaneously run the system 5 times with different seeds. 
Our transfer attack to both GAL and ReFeX consists of four steps: \textit{data pre-processing}, \textit{targets identification}, \textit{graph poisoning} and \textit{evaluation}. 

\subsubsection{Data pre-processing}
%In \textit{data preprocessing} part, 
$\mathsf{OddBall}$ operates in an unsupervised setting while both GAL and ReFeX are supervised methods. We thus pre-process the data by assigning anomaly labels to a set of nodes. Specifically, given a graph, we first use $\mathsf{OddBall}$ to compute the anomaly scores for all the nodes and label those nodes with high anomaly scores as anomalous. We then randomly split the nodes into training and testing sets.
\subsubsection{Targets identification}
As $\mathsf{BinarizedAttack}$ is a targeted attack, the goal of our transfer attack is not to decrease the prediction accuracies of the GAD systems. Instead, we are interested in changing the prediction results of a set of nodes -- those nodes that are initially predicted as anomalous by the GAD systems.
Thus, we feed the pre-processed data into GAL or ReFeX and obtain the predicted labels of the test nodes and pick those nodes \textit{predicted as anomalous} as our attack targets. 
\subsubsection{Graph poisoning} With the targeted nodes identified from the previous step, we directly use $\mathsf{BinarizedAttack}$ to generate a poisoned graph. We emphasize that the attack occurred in a black-box setting, where we do not need any information from GAL nor ReFeX.

\subsubsection{Evaluation} We provide the clean graph and poisoned graph separately as input to GAL and ReFeX. We evaluate the performance of transfer attack mainly from two aspects: 1) whether the target nodes can successfully evade the detection of GAL or ReFeX; 2) the changes of node embeddings generated by GAL and ReFeX before and after attack. 

We present the detailed experiment settings and results in Section~VIII.



%For a given graph, we firstly determine the anomaly labels by $\mathsf{AScores}$ histogram provided by $\mathsf{OddBall}$. We set those nodes whose $\mathsf{AScores}$ are located at tail of distribution as anomaly. We then split the whole dataset into training and testing data. In \textit{targets construction} part, we feed the clean graph to representation learning models (GAL or ReFeX) and obtain the embeddings for each node. We further feed the MLP with training data and testing data to measure the quality of the embeddings for the node anomaly detection task. We then determine those nodes predicted as anomaly by MLP as our target nodes for $\mathsf{BinarizedAttack}$. In \textit{poisons generation} part, we implement $\mathsf{BinarizedAttack}$ on the target nodes to generate poisoned graphs under different budget constraints $b\in\{1,2,...,B\}$. In the final part, for each $b$, we feed the poisoned graph to the representation learning model (GAL or ReFeX) and get the poisoned embeddings. We further train MLP with poisoned training data and report the quality of embeddings for target nodes. The whole tranfer attack is implemented in black-box manner.

%In order to cogently measure the attack transferability of $\mathsf{BinarizedAttack}$ to the representation learning model for node anomaly detection, we instead focus on the \textit{soft labels} \cite{hinton2015distilling} provided by the classifiers for each target node. In the representation learning, the sum of \textit{soft label} for target nodes is defined as: $\sum_{i=1}^{K}P_{i}(Y_{i}=1|\theta)=\sum_{i=1}^{K}f_{\theta}(X_{emb})$, where $\theta$ is the weight of MLP, $f(\cdot)$ is MLP, $X_{emb}$ is the node embeddings created by GAL or ReFeX. Refer to \cite{hinton2015distilling}, \textit{soft labels} have high entropy which provide much more information than hard label. So \textit{soft label} can capture the quality of embeddings in this scenario more precisely. We further implement the dimension reduction method like t-SNE \cite{tsne} to visualize the penultimate hidden features of MLP on the testing set in 2-D space. Refer to \cite{DBLP:journals/corr/abs-1808-05385} the penultimate hidden features of the MLP will form the linear separable space in 2-D space after dimension reduction (PCA \cite{pca} or t-SNE \cite{tsne}). The 2-D scatterplot will capture the effect of $\mathsf{BinarizedAttack}$ to the anomaly detection based representation learning method.

%\subsubsection{Trasnfer attack to GAL}
%GAL is an error-bounded margin loss especially designed for the anomaly detection tasks for GNNs. It captures the node similarity using the global grouping patterns discovered from the graph mining algorithms. In order to solve the imbalanced problem in anomaly detection, GAL can automatically adjust the margins for the minority class. The framework of GAL is the combination of GNNs and the error-bounded loss function. GAL replace the softmax loss of GNN to graph anomaly loss:

%\begin{align}
%	\mathcal{L}(u)=&E_{u_{+}\sim \mathcal{U}_{u+},u_{-}\sim \mathcal{U}_{u-}} max\{0,g(u,u_{-})-g(u,u_{+})+\Delta_{y_{u}}\} \nonumber \\
%	&where \quad \Delta_{y_{u}}=\frac{C}{n_{y_{u}}^{1/4}}. \label{eqn-gal}
%\end{align}
%$\mathcal{U}_{u+}$ denotes the set of nodes have the same label of node $u$ and vice versa. Here we focus on \textit{GraphSAGE} with error-bounded loss to the anomaly detection task. In transfer attack framework, we firstly use $\mathsf{BinarizedAttack}$ on real datasets ({Bitcoin-Alpha} and {Wikivote}) and generate the poisoned graphs under different attacking levels. Secondly we implement the $\mathsf{OddBall}$ to calculate the anomaly scores ( from now on for simplicity we denote anomaly score as $\mathsf{AScore}$) for each node in the graph. We then determine the anomaly labels by assigning the threshold based on $\mathsf{AScore}$ histogram and let those nodes whose $\mathsf{AScore}$ is larger than the pre-defined threshold as anomaly. Next we split the graph and create training and testing dataset and apply GAL to construct the embeddings for each node trained on \textit{GraphSAGE} with graph error-bounded loss. We implement the MLP with default structure in \cite{10.1145/3340531.3411979} to check whether deep learning model is trained sufficiently enough. We determine the target nodes for $\mathsf{BinarizedAttack}$ as those nodes predicted as anomaly in the testing dataset. In the attacking procedure, we implement $\mathsf{BinarizedAttack}$ on the target nodes under different buedget constraints. In the experiment we use the soft label for each node provided by MLP to measure the attack transferability from $\mathsf{BinarizedAttack}$ to GAL. The soft label for target nodes is defined as $\sum_{i=1}^{K}P_{i}(Y_{i}=1)=\sum_{i=1}^{K}f_{\theta}(X_{emb})$, where $f_{\theta}$($\cdot$) is MLP, $X_{emb}$ is the embeddings provided by GAL for target nodes. 
%\subsubsection{Transfer attack to ReFeX}



